Multimodal Maximum Entropy Dynamic Games

Environments with multi-agent interactions often result a rich set of modalities of behavior between agents due to the inherent suboptimality of decision making processes when agents settle for satisfactory decisions. However, existing algorithms for solving these dynamic games are strictly unimodal and fail to capture the intricate multimodal behaviors of the agents. In this paper, we propose MMELQGames (Multimodal Maximum-Entropy Linear Quadratic Games), a novel constrained multimodal maximum entropy formulation of the Differential Dynamic Programming algorithm for solving generalized Nash equilibria. By formulating the problem as a certain dynamic game with incomplete and asymmetric information where agents are uncertain about the cost and dynamics of the game itself, the proposed method is able to reason about multiple local generalized Nash equilibria, enforce constraints with the Augmented Lagrangian framework and also perform Bayesian inference on the latent mode from past observations. We assess the efficacy of the proposed algorithm on two illustrative examples: multi-agent collision avoidance and autonomous racing. In particular, we show that only MMELQGames is able to effectively block a rear vehicle when given a speed disadvantage and the rear vehicle can overtake from multiple positions.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> paper/data_table.tex <==
\begin{table*}[t]
    \centering
    \caption{Comparisons of mean and standard deviation of cost against \ac{MPPI} and \ac{CEM} on different systems and policy classes. The policy classes are defined as Unimodal Gaussian (UG), Gaussian Mixture (GM), and Stein (S). Note that the negative of the reward is used for the locomotion tasks (ant and humanoid). The best mean cost and cost variance for each system-policy distribution pair is boldfaced. The mean and standard deviation reduction percentages are included to the right where positive values correspond to a reduction.}
    \begin{tabular}{
        @{}
        l
        c
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        S[table-format=6.1,table-number-alignment = right,table-figures-decimal=1,table-auto-round]
        @{}
    }
    \toprule
    & & \multicolumn{2}{c}{MPPI} & \multicolumn{2}{c}{CEM}
    & \multicolumn{2}{c}{Tsallis} & \multicolumn{2}{c}{Tsallis vs MPPI} & \multicolumn{2}{c}{Tsallis vs CEM}\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
    {System} & {Policy} & {Mean} & {Std} & {Mean} & {Std} & {Mean} & {Std} &
    {$\Delta$Mean\%} &
    {$\Delta$Std\%} &
    {$\Delta$Mean\%} &
    {$\Delta$Std\%} \\
    % % End of header row.
    % ======== Planar Navigation ========
    \midrule
    \multirow{3.8}{*}{\begin{tabular}[c]{@{}c@{}}Planar\\Navigation\end{tabular}}
    & \begin{tabular}[c]{@{}c@{}} UG \\ \end{tabular} &
    30023.73 & 3644.07 & 34617.47 & 2523.34 & \bfseries 28714.74 & \bfseries 570.23 & 4.36 & 84.35 & 17.05 & 77.40 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM \\ \end{tabular} &
    39313.84 & 8924.76 & 53385.30 & \bfseries 5493.97 & \bfseries 31369.22 & 5683.23 & 20.21 & 36.32 & 41.24 & -3.44 \\
    \cmidrule(l){2-12} 
    & S & 38224.95 & 5169.92 & 38847.56 & 6641.78 & \bfseries 33324.48 & \bfseries 4006.43 & 12.82 & 22.50& 14.22 & 39.68 \\
    % ======== Quadcopter ========
    \midrule
    \multirow{3.8}{*}{Quadcopter}
    & \begin{tabular}[c]{@{}c@{}}UG \\\end{tabular} &
    15266.15 & \bfseries 1374.04 & 15756.75 & 2707.08 & \bfseries 14673.40 & 1458.36 & 3.88 & -6.14 & 6.88 & 46.13 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM \\\end{tabular} &
    22145.51 & 4007.33 & 17654.08 & 1593.86 & \bfseries 16430.56 & \bfseries 1498.24 & 25.81 & 62.61 & 6.93 & 6.0 \\
    \cmidrule(l){2-12} 
    & S &
    29238.25 & 5084.31 & 21064.73 & 2218.02 & \bfseries 15976.02 & \bfseries 1218.32 & 45.36 & 76.04 & 24.16 & 45.07 \\
    % ======== Manipulator ========
    \midrule
    \multirow{3.8}{*}{Franka}
    & \begin{tabular}[c]{@{}c@{}}UG \\\end{tabular} &
        64.17 & 8.43 & 66.37 & 18.40 & \bfseries 57.41 & \bfseries 5.53 & 10.6 & 34.5 & 13.6 & 70.1 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM \\\end{tabular} &
        67.16 & 8.26 & 68.74 & 13.01 & \bfseries 59.15 & \bfseries 5.37 & 11.98 & 34.9 & 13.90 & 58.5 \\
    \cmidrule(l){2-12} 
    & S & 72.40 & 4.22 & 80.35 & 13.96 & \bfseries 71.77 & \bfseries 3.29 & 0.8 & 21.4 & 10.7 & 76.4 \\
    % ======== Ant ========
    \midrule
    \multirow{3.8}{*}{Ant}
    & \begin{tabular}[c]{@{}c@{}}UG\\ \end{tabular} &
        -528.7 & 54.1 & -652.6 & \bfseries 26.7 & \bfseries -692.9 & 37.2 & 31.1 & 31.3 & 6.2 & -39.0 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM \\ \end{tabular} &
        -621.0 & 55.5 & -659.1 & 53.6 & \bfseries -663.8 & \bfseries 36.3 & 6.9 & 34.7 & 0.7 & 32.4 \\
    \cmidrule(l){2-12} 
    & S &
        -673.7 & 36.1 & -670.0 & 32.2 & \bfseries -677.4 & \bfseries 13.4 & 0.6 & 62.8 & 1.1 & 58.3 \\
    % ======== Humanoid ========
    \midrule
    \multirow{3.8}{*}{Humanoid}
    & \begin{tabular}[c]{@{}c@{}}UG\\ \end{tabular} &
        -423.79 & 233.81 & -660.80 & 208.48 & \bfseries -899.27 & \bfseries 80.09 & 112.20 & 65.74 & 36.09 & 61.58 \\
    \cmidrule(l){2-12} 
    & \begin{tabular}[c]{@{}c@{}}GM\\ \end{tabular} &
        -592.85 & 170.15 & -725.92 & 164.92 &\bfseries -738.08 & \bfseries 103.76 & 24.50 & 39.02 & 1.67 & 37.09 \\
    \cmidrule(l){2-12} 
    & S &
        -794.69 & 173.96 & -840.81 & 168.12 & \bfseries -919.67 & \bfseries 105.85 & 15.73 & 39.15 & 9.38 & 37.04 \\
    \bottomrule
    \end{tabular}
    \label{tab:data_table}
\end{table*}

==> paper/old_mme_sections.tex <==
\section{Multimodal Maximum Entropy Dynamic Games}
\label{sec:mme}
While Maximum Entropy LQGames can model inexactness in the control, it does so via a unimodal Gaussian approximation which may not be flexible enough in cases where the true value function
is not unimodal.
This is a common situation that can arise from nonconvex dynamics, nonconvex cost functions or nonconvex state constraints such as collision avoidance.
In this section, we derive a multimodal extension to MELQGames to address this problem.

% For example, consider the following simple single-agent single-timestep single-integrator unconstrained dynamic game (i.e. an optimal control problem):
% \begin{align}
%     x^1_{1} = x^1_0 + u^1
% \end{align}
% (Some $\exp(-10x^2) + u^2$ thing. Doesn't really make sense as a game maybe? Maybe add a figure + the logsumexp approx?)
% \textbf{Should we keep this?}
% In this case, MaxEntLQGames is only able to model one of the two modes. In this section, we derive a multimodal extension to MaxEntLQGames

Let $\{ \bar{\vx}^{a}, \bar{\vu}^{a} \}_{a=1}^A$ be $A$ different nominal state and control trajectories and
let $\Phi^{i, a}$ corresponds to the respective quadratic approximation of $\Phi^i$
around $\bar{\vx}^{a}$ and $\bar{\vu}^{a}$.
Instead of using a single quadratic approximation of $\Phi^i$ for the terminal cost as in \eqref{eq:me:term_quad}, we use the following combined approximation $\tilde{\Phi}$
\begin{equation} \label{eq:mme:logsumexp_Phi}
\tilde{\Phi}^i( \vx_T ) \coloneqq
    -\alpha \ln \sum_{a=1}^A \exp \left(
        -\frac{1}{\alpha} \Phi^{i,a}( \vx_T )
    \right).
\end{equation}
The log-sum-exp is a smoothed combination of the local quadratic approximation and approaches $\min_n \{ \Phi^{(n)} \}$ as $\alpha$ approaches $0$,
as shown in \cref{fig:mme:logsumexp}.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/logsumexp.pdf}
    \caption{Comparison of the individual quadratic approximation (top) and the
    log-sum-exp approximation (bottom) of the cost function $l(x)$ with varying
    choices of inverse temperature $\alpha$.
    Higher values of $\alpha$ result in a smoother approximation of $l$.}
    \label{fig:mme:logsumexp}
\end{figure}

Now, define $\expalph$ to be the following function:
\begin{equation}
    \expalph(y) \coloneqq \exp \Big(-\frac{1}{\alpha} y\Big).
\end{equation}
Then, since $V^i = \Phi^i$ at the final timestep,
\begin{align}
    z_T^i(\vx)
    &= \expalph(V^i) = \sum_{a=1}^A \expalph(\Phi^{i,a}(\vx)) \\
    &= \sum_{a=1}^A r^{i, a}_T(\vx)
\end{align}
Now, define $z_T^{i,a}(\vx) \coloneqq r^{i, a}_T(\vx)$ such that
\begin{equation}
    z_T^i(\vx) = \sum_{a=1}^A z_T^{i,a}(\vx)
\end{equation}
With this choice of $z^{i}_T$, Bellman's equation \eqref{eq:dp:linear_bellman} at time $T-1$ takes the form
\begin{align}
    z^i_{T-1}(\vx)
    &= \int {q^i}'(\vx, \ui) \, r^i(\vx, \ui) \; \dui \\
    &= \int \expalph\left( \ExP{\vunegi}{ {V'}^i( f(\vx, \vu) ) }\right)
\end{align}

This additive structure of $z^i$ is preserved when recursively applying Bellman's equation, as shown in the following lemma.
\todo{Define ${q^{i,a}}'$ somewhere.}
\begin{lemma}
    Define the desirability function $z^{i,a}$ for mode $a$ as 
    \begin{equation}
        z^{i, a}(\vx) = \int (q^{i,a})'( \vx, u^i ) r^i(\vx, u^i) \dui
    \end{equation}
    Then, 
    \begin{equation}
        z^{i}(\vx) = \sum_{a=1}^A z^{i, a}(\vx)
    \end{equation}
\end{lemma}
\begin{proof}
Suppose that ${q^i}'(\vx, \ui) = \sum_{a=1}^A {q^{i, a}}'(\vx, \ui)$.
Then, 
\begin{align}
    z^i(\vx)
    &= \int {q^i}'(\vx, u^i) r^i(\vx, u^i) \dui \\
    &= \int \left( \sum_{a=1}^A {q^{i, a}}'(\vx, u^i) \right) r^i(\vx, u^i) \dui \\
    &= \sum_{a=1}^A \int {q^{i, a}}'(\vx, u^i) r^i(\vx, u^i) \dui \\
    &= \sum_{a=1}^A z^{i, a}(\vx) \label{eq:mme:compose_valuefn}
\end{align}
\end{proof}
We now show that the optimal policy for the $i$th agent is \textit{bilinear} in $(\tilde{z}')^i$ and $r^i$.
\begin{lemma} \label{lemma:linear_policy}
The optimal policy $\pi^i$ for the $i$th agent has the form
\begin{equation}
    \pi^{i*}(u^i) = {Z^i}^{-1} \; (\tilde{z}')^{i}( \vx, u^i ) \, r^i( \vx, u^i )
\end{equation}
\end{lemma}
\begin{proof}
\begin{align}
\pi^{i*}(u^i)
&= {Z^i}^{-1} e^{\left( -\int \pi^{\negi}(\vunegi) \left[ l^i(\vx, \vu) + {V'}^i( f(\vx, \vu) ) \right] \dif \vunegi \right) } \\
&= {Z^i}^{-1} e^{-\ExP{\vunegi}{ l^i(\vx, \vu) }} \, e^{-\ExP{\vunegi}{{V'}^i( f(\vx, \vu) } } \\
&= {Z^i}^{-1} \; (\tilde{z}')^{i}( \vx, u^i ) \, r^i( \vx, u^i )
\end{align}
\end{proof}
Using the above, assuming the desirability function can be represented as a sum of individual desirability functions, the following lemma show that the optimal policy is a mixture distribution of the policies corresponding to the individual desirability functions:
\begin{lemma}
Suppose that $z^i(\vx) = \sum_{a=1}^A z^{i, a}(\vx)$.
Then,
\begin{equation}
    \pi^{i*}(\ui|\vx) = \sum_{a=1}^A w^{i, a}(\vx) \pi^{i, a}(\ui | \vx)
\end{equation}
where
\begin{align}
    w^{i, a}(\vx) &\coloneqq \frac{z^{i, a}(\vx)}{ z^{i}(\vx) }, \label{eq:mme:weights} \\
    \pi^{i, a}(\ui | \vx) &\coloneqq z^{i, a}(\vx)^{-1} \, (\tilde{z}')^{i, a}(\vx, \ui) \, r^i( \vx, \ui ).
\end{align}
In particular, $\pi^{i, a}$ is exactly the optimal policy from only considering the $a$th component $z^{i, a}$ from \cref{lemma:linear_policy}.
\end{lemma}
\begin{proof}
Using \cref{lemma:linear_policy} and that $Z^i(\vx) = z^i(\vx)$:
\begin{align}
    \pi^i( \ui | \vx )
    &= {z^i}(\vx)^{-1} \; (\tilde{z}')^{i}( \vx, \ui ) \, r^i( \vx, \ui ) \\
    &= {z^i}(\vx)^{-1} \; \left(\sum_{a=1}^A (\tilde{z}')^{i, a}( \vx, \ui ) \right) \, r^i( \vx, \ui ) \\
    &= \sum_{a=1}^A \frac{ z^{i, a}(\vx) }{ z^i(\vx) } z^{i, a}(\vx)^{-1}
        (\tilde{z}')^{i, a}( \vx, \ui ) \, r^i( \vx, \ui ) \\
    &= \sum_{a=1}^A w^{i, a}(\vx) \, \pi^{i, a}(\ui | \vx) \label{eq:mme:compose_policy}
\end{align}
\end{proof}
Since each $V^{i, a} = -\ln( z^{i, a} )$ is quadratic in $\vx$ and we have taken quadratic approximations of the costs, each $\pi^{i, a}$ will hence be Gaussian as before.
Note that the weights $w^{i,a} = \frac{}{} = \frac{}{}$ is the softmax function applied to the the value functions for each mode $a$.
Additionally, since each $V^{i,a}_t$ is a quadratic approximation of the value function dependent on $\vx_t$, the resulting weights $w^{i,a}_t$ will also depend on the $\vx_t$.
As a result, the weights $w^{i,a}_t$ are not constant and implicitly depend on the controls $\vu_{0:t-1}$ from earlier timesteps through $\vx_t$.
% Also, since $V^{i,a}$ is positive semidefinite, $z^{i, a}$ can be interpreted as a kind of ``nearest-neighbor'' weight, where trajectories closer to the the mode will be weighted higher if the nominal value function is low enough.

Finally, since both $z^i$ and $\pi^i$ are weighted sums of $z^{i, a}$ and $\pi^{i, a}$,
computing the solution to the backward pass of of MMELQGames is equivalent to solving for MELQGames around the
$A$ different nominal trajectories and then \textit{composing} the value functions and policies via \eqref{eq:mme:compose_valuefn} and \eqref{eq:mme:compose_policy}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Latent Mode Bayesian Inference via MaxEnt}
\label{sec:inference}
One advantage of the MaxEnt approach is that we obtain a policy distribution over controls $\pi(\ui|\vx)$ for all agents.
This property is exploited in MaxEnt IRL approaches, where we can perform inference on cost functions by minimizing the KL divergence between this induced policy distribution and data.
In contrast, we make use of this to perform online Bayesian inference on the latent mode $a$ for other agents using the previous controls of the other agents.

We consider a Bayesian approach and assume that the latent mode variable $a$ is fixed in time and has probability equal to the weight of mode $a$ in agent $i$'s stochastic policy at time $t=1$ \eqref{eq:mme:weights}:
\begin{equation}
    p^i(a|\vx_1)
    = \frac{ z^{i,a}(1, \vx_1) }{ z^{i}(1, \vx_1) }
    = \softmax\left( -\frac{1}{\alpha} V^{i,a}(1, \vx_1) \right)
\end{equation}
Also, we assume that the all agents observe the same value of the latent variable $a$.
Suppose that the controls of other agents $\vunegi_0$ is observed. Then,
\begin{equation} \label{eq:inference:mode}
    p(a | \vunegi_0, \vx_0, \vx_1)
    = \frac{ p(\vunegi_0 | \vx_0, a) \; p^i(a|\vx_1) }{ \sum_{b} p(\vunegi_0|\vx_0, b) \; p^i(b|\vx_1) }
\end{equation}
where $p(\vunegi_0|\vx_0, a)$ is Gaussian from \eqref{eq:me:opt_pol}.

The above is equivalent the solution to the following MaxEnt problem for $p(a|\vu_0, \vx_0)$:
\begin{align}
    \argmin_{p} \ExP{a \sim p}{ \sum_i Q^{i,a}(0, \vx_0, \vu_0) } - H[p]
\end{align}
The optimal distribution for $p(a | \vu_0, \vx_0)$ then has the form
\begin{align}
    &\phantom{{}={}} p^*(a | \vu_0, \vx_0) \\
    &= \frac{\exp(-\sum_i Q^{i, a}(0, \vx_0, \vu_0))}
        {\sum_{b} \exp(-\sum_i Q^{i, b}(0, \vx_0, \vu_0)) } \\
    % &= \frac{\exp(-Q^{\negi, a}(0, \vx_0, \vu_0)-Q^{i, a}(0, \vx_0, \vu_0) )}
        % {\sum_{b} \exp(-Q^{\negi, b}(0, \vx_0, \vu_0)-Q^{i, b}(0, \vx_0, \vu_0)) } \\
    &= \frac{\exp(-Q^{\negi, a}(0, \vx_0, \vu_0))\exp(-Q^{i, a}(0, \vx_0, \vu_0) )}
        {\sum_{b} \exp(-Q^{\negi, b}(0, \vx_0, \vu_0)) \exp(-Q^{i, b}(0, \vx_0, \vu_0)) } \\
    %
    &= \frac{\exp(-Q^{\negi, a}(0, \vx_0, \vu_0))\exp(-V^{i, a}(1, \vx_1) )}
        {\sum_{b} \exp(-Q^{\negi, b}(0, \vx_0, \vu_0)) \exp(-V^{i, b}(1, \vx_1)) } \\
    %
    &= \frac{ p(\vunegi_t|a, \vx_0) \; p^i(a | \vx_1) }{ \sum_{b} p(\vunegi_t|b,\vx_0) \; p^i(b | \vx_1) }
\end{align}
Where the second last line follows from $l^{i,a}(0, x, u) = l^{i,b}(0,x,u)$.

With $p(a | \unegi_0, \vx_0, \vx_1)$, we can now obtain $p(\ui_1 | \unegi_0, \vx_0, \vx_1)$ via
\begin{equation} \label{eq:inference:control}
    p(\ui_1 | \unegi_0, \vx_0, \vx_1) = \sum_{a=1}^A p(\ui_1 | a, \vx_1) p(a | \unegi_0, \vx_0, \vx_1)
\end{equation}
where $p(\ui_1 | a, \vx_1)$ is similarly Gaussian from \eqref{eq:me:opt_pol}.

This suggests an approach of combining the game-theoretic planning from MELQGames with mode inference: instead of planning from the current timestep, we instead plan from the \textit{previous} timestep to obtain a multimodal stochastic policy for each agent.
We can then use \eqref{eq:inference:mode} to infer a distribution on $a$ and hence compute the posterior on $p(\ui_1)$ using \eqref{eq:inference:control}.
